Arcs on Punctured Disks Intersecting at Most Twice with Endpoints on the Boundary

Let $D_n$ be the $n$-punctured disk. We prove that a family of essential simple arcs starting and ending at the boundary and pairwise intersecting at most twice is of size at most $\binom{n+1}{3}$. On the way, we also show that any nontrivial square complex homeomorphic to a disk whose hyperplanes are simple arcs intersecting at most twice must have a corner or a spur.

==> Prop_From_Theorem.tex <==
In this section, we show how Proposition~\ref{Cloud_Prop} 
follows from Theorem~\ref{Square_Cplx_Thm}. 
\begin{Definition}
  Let $\mc{A}$ be a good family of arcs as in 
  Proposition~\ref{Cloud_Prop}. After a small 
  perturbation, we can assume that there are no triple 
  intersections of arcs in $\mc{A}$. Consider the square 
  complex, $X(\mc{A})$, \emph{dual} to $\mc{A}$. Each vertex 
  in $X(\mc{A})$ corresponds to a connected component of 
  $D_n\ssm \cup \mc{A}$, and edges correspond to arc segments 
  in the boundary of adjacent components. 
\end{Definition}
\begin{Remark}
  If $\mc{A}$ is any family of arcs starting and ending 
  at $\del D_n$, then $X(\mc{A})$ is homotopy equivalent to 
  a disk through the detract of $\del D_n$ to $\del X(\mc{A})$, as in 
  Figure~\ref{fig:Square_Complex_Retract}
    \begin{center}
      \begin{figure}
        \includegraphics[width=0.3\linewidth]{Square_Complex_Retract.png}
        \caption{A retraction from $\del D_3$ to $\del X(\mc{A})$ 
        where $\mc{A}$ is a maximal good family.}
        \label{fig:Square_Complex_Retract}
      \end{figure}
    \end{center}
\end{Remark}

Why this square complex is homotopy equiv. to a disk. Show retraction 
from $\del D_n$ to $X$. Picture will suffice.

\begin{Lemma} \label{Corner_Max}
  \begin{enumerate}
    \item If $X(\mc{A})$ has a spur, then $\mc{A}$ has an isolated arc. 
    \item If $X(\mc{A})$ has a corner, then $\mc{A}$ is not maximal.
  \end{enumerate}
\end{Lemma}
\begin{proof}
  \begin{enumerate}
    \item A spur corresponds to a region $A$ that is adjacent to a 
      single other region $B$ along a single arc $\alpha$. This 
      means that $\del A \cap \del B=\alpha$, and thus, 
      $\alpha$ is disjoint from any other arc in $\mc{A}$, 
      since $A,B$ are toppological disks. Since $\alpha$ is essential, 
      both $A$ contains at least one puncture, and since $X(\mc{A})$ has a 
      spur terminating at $A$, it follows that $\mc{A}\ssm \alpha$ 
      is contained in $B$. If $A$ has at least two punctures, this 
      contradicts maximality of $\mc{A}$ (see 
      Figure~\ref{fig:Spur_Side_Punctures})
  \begin{center}
    \begin{figure}
      \includegraphics[width=0.4\linewidth]{Spur_Side_Punctures.png}
      \caption{The region $A$ cannot contain more than one puncture, or 
      else the arc $\beta$ in the figure could be added to $\mc{A}$.}
      \label{fig:Spur_Side_Punctures}
    \end{figure}
  \end{center}
    \item Let $e_1,e_2$ be the edges forming the corner at vertex $v$ in 
      $X(\mc{A})$, and let $w_1=[e_1],w_2=[e_2]$ be their respective walls. 
      Consider the region in $D_n\ssm \cup \mc{A}$ corresponding to $v$, 
      call it $A_v$ (see Figure~\ref{fig:Corner_Contradicts_Min}).
  \begin{center}
    \begin{figure}
      \includegraphics[width=0.4\linewidth]{Corner_Contradicts_Min.png}
      \caption{The region $A$ cannot contain more than one puncture, or 
      else the arc $\beta$ in the figure could be added to $\mc{A}$.}
      \label{fig:Corner_Contradicts_Min}
    \end{figure}
  \end{center}
      If $A_v$ does not contain a puncture, then the arcs 
      corresponding to $w_1,w_2$ will not be in minimal position. If 
      $A_v$ does contain a puncture, then the arc $\del A_v\ssm (\del D_n)$ 
      is disjoint from all other arcs in $\mc{A}$, and is good, and thus, 
      $\mc{A}$ is not maximal.
  \end{enumerate}
\end{proof}
\begin{proof} [Proof of Proposition~\ref{Cloud_Prop} from 
  Theorem~\ref{Square_Cplx_Thm}]
  If $\mc{A}$ has an isolated arc, then we are done. Otherwise, 
  $X(\mc{A})$ has a corner or a spur, and hence, 
  by Lemma~\ref{Corner_Max}, $\mc{A}$ is not maximal, 
  giving a contradiction.
\end{proof}


